PDE-LEARN: Using Deep Learning to Discover Partial Differential Equations from Noisy, Limited Data

In this paper, we introduce PDE-LEARN, a novel deep learning algorithm that can identify governing partial differential equations (PDEs) directly from noisy, limited measurements of a physical system of interest. PDE-LEARN uses a Rational Neural Network, $U$, to approximate the system response function and a sparse, trainable vector, $\xi$, to characterize the hidden PDE that the system response function satisfies. Our approach couples the training of $U$ and $\xi$ using a loss function that (1) makes $U$ approximate the system response function, (2) encapsulates the fact that $U$ satisfies a hidden PDE that $\xi$ characterizes, and (3) promotes sparsity in $\xi$ using ideas from iteratively reweighted least-squares. Further, PDE-LEARN can simultaneously learn from several data sets, allowing it to incorporate results from multiple experiments. This approach yields a robust algorithm to discover PDEs directly from realistic scientific data. We demonstrate the efficacy of PDE-LEARN by identifying several PDEs from noisy and limited measurements.

==> Extra.tex <==

\subsection{Heat Equation (2D)} \label{sub_sec:Heat}

Next, we consider the Heat equation in two spatial dimensions, a linear second order PDE.
The heat equation, first discovered by Joseph Fourier in 1822, describes the how heat diffuses through a given object. 
With two spatial dimensions, the heat equation takes the following form: 

\begin{equation} D_{t} U = -\alpha \Delta U = \alpha \left( D_{x}^2 U + D_{y}^2 U \right) \label{eq:Heat} \end{equation}

Where $\alpha > 0$ is a constant known as the \textit{diffusivity constant}.
Here, temperature, $U$, is a function of $x$, $y$, and $t$.

\bigskip

We test \texttt{PDE-LEARN} on a data set for the heat equation with $\alpha = .1$ on the domain $(t, x, y) \in [0, 5] \times [-5, 5] \times [-5, 5]$. 
For this data set,

$$U(0, x, y) = -\exp\left( -\frac{(x^2 + y^2)}{4} \right)\cos(xy).$$

To make the data set, we partition the problem domain into a spatiotemporal grid with $65$ grid lines along the $x$ and $y$ axis, and $101$ along the $t$ axis. 
We use \texttt{spin2} function in \texttt{chebfun} \cite{driscoll2014chebfun} to evaluate the solution at each grid point in this grid. 
The script \texttt{Heat\_Exp\_Cos\_2D.m} in the \texttt{MATLAB} sub-directory of our repository generates this data set.

\bigskip 

We use the 2D heat equation data set to generate four training data sets at four different noise levels: $25\%$, $75\%$, $75\%$, and $100\%$.
We create each data set using the procedure outlined at the beginning of section \ref{sec:Experiments}.
Each data set contain $10,000$ data points/samples. 
 
\bigskip 

We test \texttt{PDE-LEARN} on both data sets.
In all both cases, our library functions consist of all polynomial library functions of degree $\leq 2$ ($J = 2$)  whose constitute terms are in $\{ U, D_x U, D_x^2 U \}$ ($M = 3$).
We also use $5,000$ Collocation points.
We train $U$ and $\xi$ for $1000$ epochs using the Adam optimizer \cite{kingma2014adam} with a learning rate of $0.001$. 
During this portion of the training, $\lambda = 0$. 
For the $25\%$ noise data set, we subsequently set $\lambda = 0.0001$ and train for $100$ epochs using the LBFGS optimizer \cite{liu1989limited} with a learning rate of $0.1$. 
For the $50\%$ noise data set, we set $\lambda = 0.0004$ and train for $100$ epochs of LBFGS with a learning rate of $0.1$. 
Finally, for the $75\%$ and $100\%$ noise data set, we set $\lambda = 0.0005$ and train for $100$ epochs of LBFGS with a learning rate of $0.1$. 

The $25\%$ noise experiment yields the following PDE:

$$ D_t U = 0.0954(D_x^2 U) + 0.0947(D_y^2 U)$$

The $50\%$ noise experiment yields the following PDE:

$$ D_t U = 0.0893(D_x^2 U) + 0.0867(D_y^2 U)$$

The $75\%$ noise experiment yields the following PDE:

$$ D_t U = 0.0813(D_x^2 U) + 0.0785(D_y^2 U)$$

Finally, the $100\%$ noise experiment yields the following PDE:

$$ D_t U = -0.1300(U) + 0.0189(D_y U)^2$$

This final equation is not even remotely close to the heat equation.
Thus, \texttt{PDE-LEARN} successfully learns the heat equation in the first three experiments (up to $75\%$ noise), but not in the forth ($100\%$ noise).
Recall that in section \ref{sub_sec:Burgers}, \texttt{PDE-LEARN} successfully learns Burgers' equation, a non-linear PDE, at $100\%$ noise.
In general, we expect learning a non-linear PDE to be more challenging than learning a linear one, all else equal. 
That \texttt{PDE-LEARN} fails to learn the heat equation at $100\%$ noise with two spatial dimensions suggests that \texttt{PDE-LEARN} may be less resilient to sparsity and noise when training on data sets involving two spatial variables.
This makes sense, as the extra variable increases the complexity of the underlying dynamics and the number of terms that \texttt{PDE-LEARN} must identify. 
